Lower Bounds for Convexity Testing

We consider the problem of testing whether an unknown and arbitrary set $S \subseteq \mathbb{R}^n$ (given as a black-box membership oracle) is convex, versus $\varepsilon$-far from every convex set, under the standard Gaussian distribution. The current state-of-the-art testing algorithms for this problem make $2^{\tilde{O}(\sqrt{n})\cdot \mathrm{poly}(1/\varepsilon)}$ non-adaptive queries, both for the standard testing problem and for tolerant testing. We give the first lower bounds for convexity testing in the black-box query model: - We show that any one-sided tester (which may be adaptive) must use at least $n^{\Omega(1)}$ queries in order to test to some constant accuracy $\varepsilon>0$. - We show that any non-adaptive tolerant tester (which may make two-sided errors) must use at least $2^{\Omega(n^{1/4})}$ queries to distinguish sets that are $\varepsilon_1$-close to convex versus $\varepsilon_2$-far from convex, for some absolute constants $0<\varepsilon_1<\varepsilon_2$. Finally, we also show that for any constant $c>0$, any non-adaptive tester (which may make two-sided errors) must use at least $n^{1/4 - c}$ queries in order to test to some constant accuracy $\varepsilon>0$.

==> sections/one-sided-adaptive-2-3-2-22-evening-safe.tex <==
%!TEX root = ../ctlb.tex


\section{One-sided adaptive lower bound}
\label{sec:one-sided-adaptive}

\begin{theorem} [One-sided adaptive lower bound, restated] \label{thm:one-sided2}
For some absolute constant $\eps>0$, any one-sided $\eps$-tester for convexity  over $N(0,I_n)$ (which may be adaptive) must use $n^{\Omega(1)}$ queries.
\end{theorem}

At a high level, the proof of \Cref{thm:one-sided} works by (1) first defining a distribution $\Dno$ of ``no-functions'' (Boolean-valued functions over $\R^n$, or equivalently, subsets of $\R^n$), and showing that an $\Omega(1)$ fraction of draws from $\Dno$ yield sets which are $\Omega(1)$-far from convex; and (2) then arguing that for a suitable absolute constant $c>0$, any $n^c$-query algorithm (even an adaptive one) has only an $o(1)$ probability of querying a set of points whose labels are inconsistent with every convex set in $\R^n$.
In the next subsection we describe the distribution $\Dno$.
 
\subsection{The distribution $\Dno$ of far-from-convex sets}

\subsubsection{Setup}

We will see that every function $f$ in the support of $\Dno$ outputs $0$
  on every input point $x\in \mathbb{R}^n$ with $\|x\|_2>\sqrt{n}$.
To describe how $f$ behaves within the $\sqrt{n}$-ball, denoted by
\[
	\Ball(\sqrt{n}):= \big\{x\in \mathbb{R}^n: \|x\|_2\le \sqrt{n}\big\},
\] 
we require some more setup.
\medskip

\noindent {\bf The Nazarov body.}
Fix $N:= 2^{\sqrt{n}}$ (we assume without loss of generality that $n$ is a perfect square, so $N$ is an integer).
\red{
For this choice of $N$, let $\bB \sim \Naz(r,N)$ where we will take $r$ to be the unique positive number such that 
	\[
		\Phi\pbra{\frac{r}{\sqrt{n}}}^N = \frac{1}{2}.
	\]
	In other words, we choose $r$ to be the unique value such that a point on the boundary of $\Ball(\sqrt{n})$ has probability $1/2$ of being in $\bB \sim \Naz(r,N)$ (cf.~\Cref{eq:nazarov-prob}). Note that  
	\[
		\Phi\pbra{\frac{r}{\sqrt{n}}} = \pbra{\frac{1}{2}}^{\frac{1}{N}} = 1 - \frac{c_1}{N}
			\quad \text{for a value~}c_1 ={\ln 2} \pm {\frac {O(1)}{N}}
	\]
	by the Taylor expansion of $e^{-\ln(2)/N}$.
}\snote{I updated this to line up with the new Nazarov section.}


\begin{figure} \label{fig:nazzy}
 \begin{center}
\includegraphics[width=0.7\textwidth]{B}
\end{center}
\caption{The Nazarov body $\bB$ (in green).  The region $\bF_1$ is shaded yellow and orange, and the orange region is $\bF_{\{1,3\}}$. }
\end{figure}

%The regions $\bF_i$ and $\bF_j$ are shaded red in Figure~1. 
%We define 
%\begin{equation} \label{eq:F}
%\bF := \bF_1 \sqcup \cdots \sqcup \bF_N
%\end{equation}
%(note that the $\bF_i$'s are disjoint), and we define 
%\begin{equation} \label{eq:Bprime}
%\bB' := \bH'_1 \cap \cdots \cap \bH'_N.
%\end{equation} 
%We will sometimes refer to $\bB'$ as the ``contracted Nazarov body''. 

  %the points of $\bB$ which are falsified by exactly those $\bH'_j$'s for which $j$ belongs to $T$, i.e.
%\begin{equation} \label{eq:DT}
%\bD_T = \cbra{x \in \bB \ : \text{~for $j \in T$ we have~}
%x \notin \bH'_j \text{~and for $j \in [N]\setminus T$ we have~}x \in \bH'_j
% }.
% \end{equation}
%Note that $\bD_{\{j\}}$ is another name for $\bF_j$, that $\bD_{\emptyset}$ is another name for $\bB'$, %and that $\bB_i = \cup_{T \ni i} \bD_T$.
%We define $\bD$ (for ``{\bf d}og ear'') to be the union of the $\bD_T$'s over all sets $T$ of size at %least two:
%\begin{equation} \label{eq:D}
%\bD := \bigcup_{|T| \geq 2, T \subseteq N} \bD_T.
%\end{equation}
%For $i \in [N]$, we further define
%\begin{equation} \label{eq:Dsuperi}
%\bD^i = \bigsqcup_{T \subset N, |T|=i} \bD_T
%\end{equation}
%to be the disjoint union of the $\bD_T$'s across all $T$ of size exactly $i$.

\medskip
\noindent {\bf The ``action directions.''} 
For each $i \in [N]$, draw a random vector $\bv^i =(\bv^i_1,\dots,\bv^i_n) \sim N(0,I_n)$ (independent of everything else).  We say that $\bv^i$ is the \emph{action direction} for the $i$-th flap $\bF_i$.

%Let's also define the 1-dimensional interval
%\[
%I := \sbra{-1/2, 1/2} \subset \R
%\]
%since we will need it soon.

\subsubsection{The distribution $\Dno$}

For a fixed setting of $\vec{H} := (H_1,\dots,H_N)$ (which also specifies $B$ and $F_i$'s) and a fixed setting of $\vec{v}:=(v^1,\dots,v^N)$, we define the function $f_{\vec{H},\vec{v}}: \R^n \to \{0,1\}$ as follows:
 
 %\rnote{Minor thing: in the previous version we had been saying, in the first line of the definition of $g_{C,\vec{H},P}$, that $g_{C,\vec{H},P}(x)$ is 0 if $\|x\|$ (not $\|x_C\|$) is outside the right range. But I think this is a little inconsistent with e.g. the second line in the definition of $g_{C,\vec{H},P}(x)$ --- it's possible for $\|x\|$ to be larger than $\sqrt{n}+10\sqrt{\ln(1/\eps)}$ but for $x$ to also lie in $B'$, if, e.g., $x$ had a freakishly large component $x_A$ (recall that $B'$ is defined only in terms of what happens in the control space, i.e. in terms of $x_C$).}

\[
f_{\vec{H},\vec{v}}(x) = \begin{cases}
0 & \text{if~} x \notin \Ball(\sqrt{n});\\
1 & \text{if~} x \in B;\\
\bigwedge_{j \in T}\Indicator\sbra{\langle v^j,x\rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]} & \text{otherwise: } x \in F_T
\text{~for some~}\emptyset \neq T \subseteq [N].
\end{cases}
\]
A random function $\boldf \sim \Dno$ is drawn as follows:  first we draw $\vec{\bH}$ as in \Cref{eq:boldH}
  and $\vec{\bv}$; then we set the function
  $\boldf$ to be $\smash{f_{\vec{\bH},\vec{\bv}}}$.

%\[
%\boldf_{\vec{H},\vec{v}}(x) = \begin{cases}
%0 & \text{if~} \|x\| > \sqrt{n}+1 ;\\
%1 & \text{if~} \|x\| < \sqrt{n}-1 ;\\
%\bg_{\vec{\bH},\vec{\bv}}(x) & \text{if~} \|x\| \in \Shell.
%\end{cases}
%\]

%\snote{The lemma on higher-order-dog-ears having small volume is now in~\Cref{sec:nazarov-prelims}.}


% ignoring old stuff
\ignore{

\subsection{Useful properties of the $\Dno$-sets}

We will require the following lemma, which states that the expected volume of $\bD^i$ decreases very rapidly as a function of $i$: {\color{red}Xi: I hope this lemma is still true, with $D^i$ now
    defined to be the union of $F_T$ for all $T$ of size $i$.}

\blue{
\begin{lemma}[Erik says maybe the following is good enough for the one-sided adaptive part] 
\label{lem:rad-by-rad}
Fix any radius $r$ we need to worry about, in $[0,\sqrt{n}]$, and fix a point $z$ with $\|z\|_2=r$.  Fix $q=n^c$ for a small constant $c$.  Then for a random Nazarov body, we have $\Pr[z \in \sqcup_{i \geq q}\bD^i] \leq O(1/q!).$  (Even a RHS of $1/4^q$ would suffice for us; this will fight a union bound over all $(1.0\cdot 2)^q$ leaves of the tree.)
\end{lemma}
}

%\begin{lemma} \label{lem:exp-decrease}
%\red{Let $m = \green{\log n}.$ For $1 \leq i \leq m$, we have
%$\sum_{j \geq i} \Ex_{\boldf \sim \Dno}[\Vol(\bD^j)] \leq O(1/i!) + 1/n$.}
%\rnote{Is this what we need? For the tolerant construction, I think we needed that $\Vol(\bD^1)$ dominates $\sum_{j\geq 2} \Vol(\bD^j)$.}


%
%Also, I think we might additionally need the statement to give us that
%$\Ex_{\boldf}[\Vol(\cup_{i \in [m+1,N]} \bD^i)]$ is not too large.}
%\end{lemma}

\red{(Mostly ignore the following since we plan to analyze the $\bD^i$'s instead of the $\bD'^i$'s)}

We provide some setup for this lemma before entering into the proof.
For $T \subseteq [N]$ define 
\[
\bD'_T := \cbra{x \in \R^n \ : \text{for each~}i \in [N], x 
\in \bS_i \text{~iff~}i \in T
},
\]
i.e.~the set of points in $\R^n$ that belong to precisely the slabs indexed by the elements of $T$.
For $T \subseteq [N]$ define 
\[
\bD'^i = \bigsqcup_{T \subset N, |T|=i} \bD'_T
\]
Note that $\bD_T=\bB \cap \bD'_T$ and $\bD'^i = \bB \cap \bD^i$.
%Hence \Cref{lem:exp-decrease} is an immediate corollary of the following:
%\begin{lemma} \label{lem:exp-decrease2}
%\red{Let $m = \green{\log n}.$ For $1 \leq i \leq m$, we have
%$\sum_{j \geq i} \Ex_{\boldf \sim \Dno}[\Vol(\bD^j)] \leq O(1/i!) + 1/n$.}
%\end{lemma}

The main idea behind \Cref{lem:exp-decrease2} is to perform the analysis on a ``radius-by-radius'' basis.
For any $t>0$, define $p_t \in [0,1]$ to be the value such that every $x \in \R^n$ with $\|x\|_2=t$ has $\Pr[x \in \bS_1]=p_t$ (this value will be the same for all $x$ with $\|x\|_2=t$ by rotational symmetry of $N(0,I_n)$).
It follows that
\begin{equation}
\label{eq:fixed-radius-t}
\text{ for $\|x\|_2=t,$ we have~}
\Pr[x \in \bD'_T]=p_t^{|T|} \cdot (1-p_t)^{N-|T|}.
\end{equation}
Let us analyze this quantity:


\bigskip\bigskip\bigskip\bigskip

\blue{create some BLAHBLAH statement roughly along the lines of the analysis in \href{https://docs.google.com/document/d/1Z45IzhgP4Ke-Y_1ZtTOfkXJ7Ewg6mR5fTJumIUtYxeI/edit}{this Google Drive file}, establishing that for any $z$ with $\|z\| = \sqrt{n}+\Delta$, where $|\Delta| \leq$ (something), we have $\Pr_{\boldf \sim \Dno}[z \in \bD'^i] = such-and-such$.  Using the fact that the variance of the $\chi^2(n)$ distribution is $2n$, we need to work out what the (something) needs to be so that we can combine the radius-by-radius bounds and only incur a small acceptable error because of outcomes of $\|\bg\|_2$ which come out outside of $[\sqrt{n}-\Delta,\sqrt{n}+\Delta]$).}

\bigskip\bigskip\bigskip\bigskip
 
With \blue{BLAHBLAH} in hand, we can bound the volume of $\bD'^i$ as follows. 
Recalling \Cref{eq:fixed-radius-t}, we have
\[
\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)]=
{N \choose i} \cdot \Ex_{\bt \sim \chi(n)}\sbra{ p_{\bt}^{i} \cdot (1-p_{\bt})^{N-i}}.
\]


\bigskip \bigskip \bigskip \bigskip \bigskip \bigskip \bigskip \bigskip 

\blue{
\subsubsection{High-order $\bD_T$'s have small volume}

\medskip

We think we will need a lemma like the following:
\begin{lemma} \label{lem:exp-decrease-old}
$\Ex_{\boldf \sim \Dno}[\Vol(\bD^i)] \leq 2^{-\Omega(i)}.$
\end{lemma}

\noindent
\emph{Proof sketch for \Cref{lem:exp-decrease}.}
We observe that $\bD_T \subseteq \bD'_T$. 
%(To see this, consider any $x \in \bD_T$. We have $x \in \bB$ so $x \in \bH_i$ for all $i \in [N]$, and $x \in \bH'_i$ for exactly those $i \in [N]$ that do not belong to $T$. Hence $x \in \bS_i$ for exactly those $i \in [N]$ that belong to $T$, so $x \in \bD'_T.$)
So to show that $\Ex_{\boldf \sim \Dno}[\Vol(\bD_i)] \leq 2^{-\Omega(i)},$ it suffices to show that $\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)] \leq 2^{-\Omega(i)}.$ 

%Recall that for $i \in [N]$ we have that slab $i$ is
%\[
%\bS_i = \bH_i \setminus \bH'_i
%\]
%(so $\bB_i \subseteq \bS_i$ because $\bS_i$, unlike $\bB_i$, may contain points that are outside of $\bB$). 


We argue that $\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)] \leq 2^{-\Omega(i)}$ by arguing radius-by-radius.  Given a real value $t > 0$, any $x \in \R^n$ with $\|x\|_2=t$ has $\Pr[x \in \bS_1]=p_t$ where $p_t = \red{BLAH}$ and hence
$\Pr[x \in \bD'_T]=p_t^{|T|} \cdot (1-p_t)^{N-|T|}$, so 
\[
\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)]=
{N \choose i} \cdot \Avg_{\bt \sim \chi(n)}\sbra{ p_{\bt}^{i} \cdot (1-p_{\bt})^{N-i}}
\]
See \href{https://docs.google.com/document/d/1Z45IzhgP4Ke-Y_1ZtTOfkXJ7Ewg6mR5fTJumIUtYxeI/edit}{this Google Drive file} for a sketch of how to prove the radius-by-radius statement or \Cref{lem:exp-decrease}.

\qed

}

} % end of ignore

\subsection{Sets in $\Dno$ are far from convex}

We need a constant fraction of the no-functions to be constant-far from convex. This is given for us by the following lemma:

\begin{lemma}  \label{lem:distance}
With probability $\Omega(1)$ over a draw of $\boldf \sim \Dno$, we have that $\Vol(\boldf  \triangle g)=\Omega(1)$ for every $g: \R^n \to \zo$ that is the indicator function of a convex set in $\R^n$.
\end{lemma}

Define $\Thinshell := \{x \in \R^n: \sqrt{n}-2 \leq \|x\|_2 \leq \sqrt{n}-1\}.$ Let us define the following two-stage random event which we denote $\bV=\bV(\boldf,\bx)$ (the randomness is over a random draw of $\boldf \sim \Dno$ and an independent random draw of $\bx \sim N(0,I_n)$; we remark that $\bV$ stands for ``violation''):

\begin{itemize}

\item In the first stage, we draw $\boldf \sim \Dno$. (This determines the $\bg^i$'s, $\bv^i$'s, $\bF_i$'s and $\bU_i$'s.)

\item In the second stage, we draw $\bx \sim N(0,I_n)$. If $x$ lies in $\bU_i \cap \Thinshell$ for some $i \in [N]$ (which must be unique), then define the vectors $\bx^+ = \bx + {\frac {\bv^i}{\|\bv^i\|}}$ and $\bx^- = \bx - {\frac {\bv^i}{\|\bv^i\|}}$.  The event $\bV=\bV(\boldf,\bx)$ holds if both (i) $\Vol((\cup_{j \in [N]} \bU_j) \cap \Thinshell)=\Omega(1)$, and (ii) $\boldf(\bx)=0$ and $\boldf(\bx^+)=\boldf(\bx^-)=1.$

\end{itemize}

Let $p := \Pr_{\boldf,\bx}[\bV].$ Our goal is to show that $p = \Omega(1)$.
To see why this suffices to give \Cref{lem:distance}, observe that if $p=\Omega(1)$ then this means that $\Ex_{\boldf}[\Pr_{\bx}[\bV(\boldf,\bx)]]=\Omega(1)$ and hence we have that $\Pr_{\bx}[\bV(f,\bx)]=\Omega(1)$  for an $\Omega(1)$ fraction of the first-stage outcomes $f$ of $\boldf$.
Fix any such first-stage outcome $f$ (which fixes the vectors $(g^j)_{j \in [N]}, (v^j)_{j \in [N]}$).  In order to ``repair'' a violation given by $x^+,x,x^-$ in the second stage, the label assigned by $f$ must be changed on at least one of those three inputs.  \red{We further observe that if $x \in U_i \cap \Thinshell$ then also $x^+,x^- \in U_i$ (because $v^i$ is orthogonal to $g^i$ and $\|x^+\|,\|x^-\| \leq \|x\|+1 \leq \sqrt{n}$).}\rnote{I think this is not true --- going from $x$ to (say) $x^+$ doesn't change membership in $\bH_i$, but it can change membership in $\bH^j$ for other values $j \neq i$. So I think it could be the case that (say) $x^+$ is now also in some other $\bF_j$, which would put it outside of $\bU_i$.}  It follows that for any two distinct points $x \in U_i \cap \Thinshell,$ $x' \in U_j \cap \Thinshell$ (here $i$ and $j$ may or may not be distinct), all six points $x^+,x,x^-,x'^+,x',x'^-$ are distinct, so all the ``violating triples'' are distinct.\snote{We might have collisions among $x^+, x, \dots$ but this should be ok: only affects us by a factor of 3. {\bf Anindya:} Actually, any point in $\R^n$ can only feature as one of $x, x^+,$ and $x^-$ so we only get a factor of $3$.}
 Next, observe that for any $x \in (\cup_{j \in [N]}\bU_j) \cap \Thinshell$ the distances $\|x-x^+\|=\|x-x^-\|$ are both $1$, and hence (using $\sqrt{n}-1 \leq \|x\| \leq \sqrt{n}$) the $\chi^2(n)$ distribution's pdf is within a constant factor on each of the three inputs $\|x\|,\|x^+\|$ and $\|x^-\|$. Combining this with $\Vol((\cup_{i \in [N]} \bU_i) \cap \Thinshell)=\Omega(1)$, we get that the value of $f$ needs to be altered on at least an $\Omega(1)$ fraction of inputs drawn from $N(0,I_n)$, which gives \Cref{lem:distance}.

We proceed to show that $p=\Omega(1).$ To show this, let $\bW$ denote the event that (i) holds; note that this depends only on the outcome of $\boldf$ in the first stage, i.e.~we have $\bW=\bW(\boldf)$.  Given an outcome $f$ of $\boldf$ such that $\bW(f)$ holds, let $\bX_f$ denote the event that (ii) holds; note that this depends only on the outcome of $\bx$ in the second stage, i.e.~we have $\bX_f=\bX_f(\bx).$ \Cref{lem:distance} follows immediately from the following two claims:

\begin{claim} \label{claim:distance1}
$\Pr_{\boldf}[\bW(\boldf)] = \Omega(1).$
\end{claim}

\begin{claim} \label{claim:distance2}
For any fixed $f$ such that $\bW(f)$ holds, we have $\Pr_{\bx}[\bX_f(\bx)] = \Omega(1).$
\end{claim}

\noindent \emph{Proof of \Cref{claim:distance1}.}
\red{FILL IN.  For this it should be enough to show that for any fixed $x$ with $\sqrt{n}-1 \leq \|x\| \leq \sqrt{n}$, we have $\Pr_{\boldf}[x \in (\cup_{j \in [N]} \bU_j)] = \Omega(1)$. What's the easiest/best way to do this given the related statements we'll need? } 
\qed

\medskip
\noindent \emph{Proof of \Cref{claim:distance2}.}
\red{FILL IN. Hopefully this one is easy?} 
\qed



%{\color{red}Xi: I hope this lemma still holds.
%\begin{claim} 
%With probability $\Omega(1)$ over a draw of $\boldf \sim \Dno$, we have that $\boldf$ is $\Omega(1)$-far from every convex set in $\R^n$ (w.r.t. Gaussian volume).
%\end{claim}
%\noindent \emph{Sketch of justification:} This follows from having $\Ex_{\boldf \sim \Dno}\sbra{\dist(\boldf,\mathrm{convex})}=\Omega(1).$ The idea for why $\Ex_{\boldf \sim \Dno}\sbra{\dist(\boldf,\mathrm{convex})}=\Omega(1)$ is roughly because (i) $\Ex_{\bH}\sbra{\Vol(\bF)}=\Omega(1)$ (this is something we will argue in the tolerant non-adaptive lower bound construction), (ii) $\Vol[\bF]=\sum_{i \in [N]}\Vol[\bF_i]$, and (iii) for a given flap $\bF_i$ we should have that (since $\bv^i$ is almost orthogonal to the direction $\bg^i$ of the hyperplane $\bH_i$ defining $\bF_i$) we can get violating triples (three points in a line segment, where the middle point is labeled 0 and the two outer points are labeled 1, and the line segment is in the direction of $\bv^i$) that in expectation cover a constant fraction of the Gaussian volume of $\bF_i$.  (This needs to be worked out in more detail but we think it should be okay.)
%% $\Ex[\Vol(\bF_i \cap \{x: |\abra{\bv^i,x}| \in [-0.5,0.5]\}] \geq \Omega(1) \cdot \Ex[\Vol(\bF_i)]$. This last property should let us argue ``line segment by line segment'' to get violating triples:  fix a segment in $\bF_i$ by specifying everything but the projection in direction $v^i$, so points on the segment vary only in their value of $\abra{x,\bv^i}.$ If there 
%\qed
%}

\subsection{Proof of \Cref{thm:one-sided}}

\newcommand{\Alg}{\mathrm{Alg}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\lsim}{\lesssim}
\newcommand{\conv}{\mathrm{conv}}

%\enote{I started going through the main structure of the argument and diving up into some lemmas. I may be mistaken on the specific events that we need, and we can hopefully discuss these on our Tuesday meeting. }

\begin{definition}[One-sided Adaptive Algorithms as Binary Trees]
Fix $n, q \in \N$. A $q$-query one-sided deterministic algorithm, $\Alg$, for testing convexity in $\R^n$ is specified by a rooted binary tree of depth $q$ where each node contains the following information:
\begin{flushleft}\begin{itemize}
\item Each node $v$ which is a not a leaf contains a query vector $x_v \in \R^n$, as well as two out-going edges, one labeled 0 and one labeled 1, to nodes which we label $v(0)$ and $v(1)$, respectively.
\item Each leaf node $v$ contains an output $o_v$ which is set to \emph{``accept''} or \emph{``reject.''} 
Let $Q_1$ (or $Q_0$) denote the set of points queried along the path that are labelled $1$
  (or $0$, respectively).
Then $o_v$ is set to be ``reject'' if and only if $Q_0\cap \conv(Q_1)\ne \emptyset$.
\end{itemize}\end{flushleft}
By adding nodes which repeat the queries, we may assume, without loss of generality, that the depth of every leaf of the tree is exactly $q$. Furthermore, we may assume without loss of generality that every $x_v$ satisfies $x_v\in \Ball(\sqrt{n})$. This is because every $y$ with $\|y\|_2 > \sqrt{n}$ must have $f(y)=0$ for every function $f$ in the support of $\Dno$, and hence such a point $y$ cannot participate in a collection of labeled points which witness that such an $f$ is not convex (i.e.~a collection of points $x_1,\dots, x_{\ell}, y$ queried by $\Alg$ with $y \in \conv(x_1,\dots, x_{\ell})$, $f(y) = 0$ and $f(x_1) = \dots = f(x_{\ell}) = 1$). 
%(Note that even though every point $x$ with $\|x\| <\sqrt{n}-1$ must have $f(x)=1$ for every $f$ in the support of $\Dno$, it may still be useful for a one-sided tester to query such points, since they can be used in constructing a witness of the $f$ non-convexity of $f$.)
%\rnote{Since this point was subtle enough to escape us before Xi noticed it, I added a quick mention for the reader.)}
  
  
\end{definition}
A $q$-query deterministic algorithm $\Alg$ executes on a function $f \colon \R^n \to \{0,1\}$ by taking the natural root-to-leaf path given by following the function values which the oracle returns at the queries within each of the nodes. In particular, we will make repeated use of the following definitions which capture the execution of the algorithm $\Alg$ on a function $f$:
\begin{flushleft}\begin{itemize}
\item The node $v^0$ is the root of the tree, which is the starting point of the root-to-leaf path. Then, the nodes $v^1,\dots, v^q$ indicate the root-to-leaf path generated by executing the algorithm on the function $f$. In particular, at time step $t \in \{ 0, \dots, q-1\}$, we have $v^{t+1} = v^{t}(f(x_{v^{t}}))$
\item The set $Q^0$ is defined to be $\emptyset$, and for $t \in \{0, \dots, q-1\}$ the set $Q^{t+1}$ is defined to be $Q^{t} \cup \{ x_{v^{t}} \} \subset \R^n$.
Thus $Q^{t+1}$ is the set of vectors that are queried at time steps prior to $t+1$.
\end{itemize}\end{flushleft}
Once the algorithm reaches the leaf node $v^{q}$, the algorithm outputs $o_{v^q}$, and we will refer to $\Alg(f)$ as the output (\emph{``accept''} or \emph{``reject''}) produced by the algorithm. It is trivial to see that since any $q$-query deterministic algorithm corresponds to a tree of depth $q$, the total number of query vectors $x_v \in \R^n$ across all nodes of the tree is at most $2^q$. Our goal is to show that, if $\Alg$ is a $q$-query deterministic algorithm which makes \emph{one-sided error}, then
\begin{align}
\Prx_{\boldf \sim \Dno}\left[ \Alg(\boldf) = \text{\emph{``reject''}}\right] = o(1).  \label{eq:adapt-final-exp}
\end{align}
Recall that implicit in a draw of $\boldf \sim \Dno$ are vectors $\bg^1,\dots, \bg^{N} \in \R^n$ and $\bv^1,\dots,\bv^{N} \in \R^n$, and that $\bg^1,\dots,\bg^N$ define $\bB$, $\bH_i$ and $\bF_i$ regions. Toward showing the above upper bound, we define two important events (which will depend on the draw $\boldf \sim \Dno$).

%Let's start with some notation.%
%Let $\Shell:=\Ball(\sqrt{n})\setminus \Ball(\sqrt{n}-100q)$.
%Next we introduce some notation for describing the execution of $\Alg$ on an $f$ 
%  from the support of $\Dno$.
%A query point $x$ along the path of running $\Alg$ on $f$ is said to \emph{discover} the %$i$th flap $F_i$
%  for some $i\in [N]$ if $x$ is the first point along the path that lies in $F_i$.
%Given a set of queries $Q$ made so far (e.g., $Q^k$ for some $k\le q$),
%  we say a flap $F_i$ is \emph{nonempty} with respect to $Q$ if $Q\cap F_i\ne \emptyset$,
%  and a nonempty flap $F_i$ is \emph{regular} if $Q\cap F_i\subset \Shell$ and 
%  every point $x\in Q\cap F_i$ satisfies 
%\begin{equation}\label{eq:hehe1}
%\langle x,g^i\rangle \le r+100qn^{1/4}.
%\end{equation}
%The motivation behind the notion of regular flaps 
%  is that, as it will become clear later in 
%  Lemma \ref{lem:ev1} (concerning the first event $\calE_1$ to be defined below),
%  it is unlikely for $\Alg$ to query a point $x$ that lands in $F_i$ for some $i$
%  and at the same time either has $x\notin \Shell$ or violates (\ref{eq:hehe1}).




%We are now ready to define the three events:

\begin{definition}
Given $\Alg$ and a function $f$ from $\Dno$, we consider the following three events:
\begin{flushleft}\begin{itemize}
\item {\color{red} $\calE_1(f)$: This event occurs 
%there exists any node $v$ within the algorithm $\Alg$ such that 
%    \begin{itemize}
%    \item either the query $x_v$ lies in the region $D^{\ge q}$ defined by $f$, or
%    \item $x_v$ satisfies $x_v\notin \Shell$ and $x_v\notin B$ (or equivalently, $x_v\in D^{\ge 1}$), or
%    \item {\color{blue}$x_v$ satisfies that $\langle x_v,g^i\rangle>r+100q n^{1/4}$ for some $i\in [N]$.}%\xnote{This is a new condition.}
%      the region $D^{\ge 1}$ defined by $f$.
%    \end{itemize}
%}
%\item {\color{red} $\calE_2(f)$: This event occurs 
if at the end of the execution of
  $\Alg$ on $f$, every point $x\in Q^q$ lies in at most $q$ flaps and
   for every flap $F_i$ with $Q^q\cap F_i\ne\emptyset$, 
  %there exist an $i\in [N]$ and two queries $x,y\in Q^q$\rnote{Minor: $Q^q$ or $Q^{q+1}$ --- isn't $Q^{q+1}$ the set of all $q$ queries the algorithm makes when the function is $f$? \color{red}Xi: Maybe it should be $Q^q$ since we start with $Q^0=\emptyset$ at the beginning.} that satisfy the following conditions:
   %produced by executing $\Alg$ on the function $f$, which satisfy the following two conditions:
%\begin{itemize}
%\item $F_i$ is among the first $q^2$ nonempty flaps with respect to $Q^q$; % $Q^q\cap F_i\ne \emptyset $;
%\item $F_i$ is regular and 
%and
 % every point $z\in Q^q\cap F_i$ satisfies $$\langle z,g^i\rangle \le r+100qn^{1/4};$$ 
%\item There exists some $i \in [N]$ where $x, y \in S_i$ \blue{and $\|x\|_2, \|y\|_2 \leq \sqrt{n} + 1$}. 
%\rnote{Do we want just the blue thing or do we want that $x,y \in \Shell$?}
} $$\|x - y\|_2 \le 500 \sqrt{q} n^{1/4},\quad\text{for all $x,y\in Q^q\cap F_i$.}$$
%\end{itemize}}
\item {\color{red}$\calE_2(f)$: This event occurs if at the end of
  the execution of $\Alg$ on $f$, for every flap $F_i$ with
  $Q^q\cap F_i\ne \emptyset$ and every $x,y\in Q^q\cap F_i$, we have }
%  there exist an $i\in [N]$ and two queries $x,y\in Q^q$ such that
%  $x,y\in F_i$ but} %$f(x)\ne f(y)$.
  $$
  \Indicator\sbra{\langle v^i , x\rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]} = \Indicator\sbra{\langle v^i,y
  \rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]}.
  $$
  % whenever there exists two queries $x, y \in Q^q$ produced by executing $\Alg$ on the function $f$ where there is some $i \in [N]$ with $x, y \in S_i$, \blue{$\|y\|_2, \|x\|_2 \leq \sqrt{n} + 1$},\rnote{Here too, do we want just the blue thing or do we want that $x,y \in \Shell$?} and $f(x) \neq f(y)$.
\end{itemize}\end{flushleft}
\end{definition}

Theorem \ref{thm:one-sided} follows immediately from the following three lemmas:

\begin{lemma}\label{lem:reject-and-3}
Let $\Alg$ be a one-sided, deterministic, $q$-query algorithm for testing convexity. Then, if $\Alg(f)$ outputs ``reject,'' the event $\overline{\calE_2(f)}$ occurred.
\end{lemma}

\begin{lemma}\label{lem:ev1}
Let $\Alg$ be a one-sided,  deterministic, $q$-query algorithm. Then,
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf)\right] \ge 1- o(1). 
\end{align*}
\end{lemma}


\begin{lemma}\label{lem:ev3}
Let $\Alg$ be a one-sided, deterministic, $q$-query algorithm, where $q \leq n^{0.1}/\log n$. Then, 
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \overline{\calE_2(\boldf)}\cap \calE_1(\boldf)\right] \le o(1).
\end{align*}
\end{lemma}

%\begin{lemma}\label{lem:ev2}
%Let $\Alg$ be a one-sided, deterministic, $q$-query algorithm, where $q \leq ??$. Then,
%\begin{align*}
% \Prx_{\boldf \sim \Dno}\left[ \calE_2(\boldf)\right]=o(1).
%%\Prx_{\boldf \sim \Dno}\left[ \calE_2(\boldf) \wedge \ol{\calE_1(\boldf)} \right] = o(1).
%\end{align*}
%\end{lemma}



\begin{proof}[Proof of Theorem~\ref{thm:one-sided} Assuming Lemmas~\ref{lem:reject-and-3}, \ref{lem:ev1} and \ref{lem:ev3}]
We upperbound the expression
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \Alg(\boldf) = \text{``accept''}\right] &\mathop{\ge}^{(\ref{lem:reject-and-3})} \Prx_{\boldf \sim \Dno}\left[ \calE_2(\boldf)\right]
\geq \Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf)\right]-
\Prx_{\boldf \sim \Dno}\left[ \overline{\calE_2(\boldf)}\cap \calE_1(\boldf)\right]\ge 1-o(1)
%  \\%
%		&\leq \Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf) \right] + \Prx_{\boldf \sim \Dno}\left[ \calE_2(\boldf) \right] + \Prx_{\boldf \sim \Dno}\left[ \calE_3(\boldf) \wedge \ol{\calE_1(\boldf)} \wedge \ol{\calE_2(\boldf)}\right],
\end{align*}
using  
  Lemmas~\ref{lem:ev1} and \ref{lem:ev3}.
\end{proof}



\subsection{Proof of Lemma~\ref{lem:reject-and-3}}

%\enote{This should be Xi's argument using the definition of convex hull, where we say that something has ``crossed the boundary''. Hopefully we can fill this in more formally...}

%\rnote{This will need to change somewhat given Xi's change to the construction}
Since $\Alg$ is a $q$-query deterministic algorithm which has one-sided error, in order for the algorithm to output ``reject,'' the set $Q^q$ queried by the root-to-leaf path obtained by executing $\Alg$ on $f$ must contain $x_1,\dots, x_{\ell}, y \in Q^q$ satisfying 
$$y \in \conv(x_1,\dots, x_{\ell}),\quad f(y) = 0,\quad \text{and}\quad f(x_1) = \dots = f(x_{\ell}) = 1.$$ In particular, from $y\in \conv(x_1,\dots,x_\ell)$, we must have that, for any vector $u \in \R^n$, there exists a $j \in [\ell]$ such that $\langle x_j, u \rangle \geq \langle y, u \rangle$. This implies that:
\begin{flushleft}\begin{itemize}
\item We must have $x_1,\ldots,x_\ell,y \in \Ball(\sqrt{n})$. The part of $x_1,\ldots,x_\ell\in \Ball(\sqrt{n})$ follows trivially from $f(x_1)=\cdots =f(x_\ell)=1$.
On the other hand, if $\|y\|_2>\sqrt{n}$, letting $u$ be the unit vector $u=y/\|y\|_2$, there exists an $x_j$ 
  with $$\langle x_j, u \rangle \geq \langle y, u \rangle =\|y\|_2> \sqrt{n},$$ and hence $\|x_j\|_2>\sqrt{n}$ and $f(x_j) = 0$, which would be a contradiction with $f(x_j)=1$.

\item We must have $y\notin B$ since $f(y)=0$.
%Otherwise there exists an $i\in [N]$ such that $\langle y,g^i\rangle >r$.
%Using $g^i$ as $u$ we have that there exists a $j\in [\ell]$ such that $\langle x_j,g^i\rangle \ge \langle y,g^i\rangle >r$, which implies that $f(x_j)=0$, a contradiction.
As a result, there is a nonempty $T$ such that $y\in F_T$.
   In addition, $f(y) = 0$ implies that 
   there exists an $i\in T$ such that $y\in F_i$ but 
   $$
   \Indicator\sbra{\langle v^i,y\rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]} = 0.
   $$
Given that $y\in F_i$, setting $u=g^i$, there exists an $x_j$ such that 
  $\langle x_j,g^i\rangle >\langle y,g^i\rangle\ge r$ and thus, $x_j\in F_i$.
It follows from $f(x_j)=1$ and the construction that %, we have 
  $$
   \Indicator\sbra{\langle v^i ,x_j\rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]} = 1.
   $$  
%    $f(y) = g_{\vec{H}, \vec{v}}(y)$ for $y \in \Shell$. In particular, there must be some index $i \in [N]$ so that $\langle x_j, g^i \rangle \geq \langle y, g^i \rangle > r - c_1 n^{1/4}$. Finally, we must have $\langle x_j , g^j \rangle \leq r$ as otherwise, $x_j \notin B$ and evaluates to $0$. For that setting of $j$, we must also have $\|x_j\|_2 \leq \sqrt{n} + 1$ since $f(x_j) = 1$. 
\end{itemize}\end{flushleft}
%In summary, we must have both $\|y\|_2, \|x_j \|_2 \leq \sqrt{n} + 1$ and $x_j, y \in S_i$ for some $i \in [N]$. 
This concludes the proof using $i,y$ and $x_j$.

\subsection{Proof of Lemma \ref{lem:ev1}}
\label{sec:proofev1}

%\begin{proof}

Let $\Shell:=\Ball(\sqrt{n})\setminus \Ball(\sqrt{n}-100q)$.
%I will be working on the non-adaptive case, where the algorithm makes
%  $2^q$ queries $Q\subset \Ball(\sqrt{n})$, where $q$ should be taken as a small polynomial of $n$.

To prove Lemma \ref{lem:ev1}, we introduce four new, easy-to-analyze events $\calE_{1,1},\calE_{1,2},
  \calE_{1,3}$ and $\calE_{1,4}$, show that each happens with probability at least $1-o(1)$,
  and that $\calE_{1,1}\cap \calE_{1,2}\cap \calE_{1,3} \cap   \calE_{1,4}$ implies $\calE_1$.
\red{\begin{flushleft}\begin{itemize}
\item $\calE_{1,1}(f)$:
This event occurs if no query $x$ in $\Alg$ lies in
  the region $D^{\ge q}$ defined by $f$;
%    \begin{itemize}
%    \item either the query $x_v$ lies in the region $D^{\ge q}$ defined by $f$, or
%    \item $x_v$ satisfies $x_v\notin \Shell$ and $x_v\notin B$ (or equivalently, $x_v\in D^{\ge 1}$), or
%    \item {\color{blue}$x_v$ satisfies that $\langle x_v,g^i\rangle>r+100q n^{1/4}$ for some $i\in [N]$.}%\xnote{This is a new condition.}
%      the region $D^{\ge 1}$ defined by $f$.
%    \end{itemize}
\item $\calE_{1,2}(f)$: This event occurs if 
  no query $x$ in $\Alg$ satisfies 
  %  $v$ in the algorithm $\Alg$ is labelled a query $x_v$ such that 
  $x\notin \Shell$  and $x\notin B$ (or equivalently, $\|x\|_2<\sqrt{n}-100q$
  and $x\in F_i$ for some $i\in [N]$);
\item $\calE_{1,3}(f)$: This event occurs if 
  no query $x$ in $\Alg$ has $$\langle x,g^i\rangle\ge r+100qn^{1/4},\quad\text{for some $i\in [N]$};$$
\item $\calE_{1,4}(f)$: This event \emph{does not} occur if 
  there exist $i\in [N]$ and two non-colinear queries $x,z$ (i.e.~$z$ is not a scalar multiple of $x$) in $\Alg$,
  where $z=(1+a)x+by$ denotes the unique decomposition with $x\perp y$, $\|y\|_2=1$ and $b>0$,
  such that $x\in F_i$ and $|\langle y,g^i\rangle |\ge 100\sqrt{q}$.
\end{itemize}\end{flushleft}}
This lemma follows from a simple union bound. Note there are at most $2^q$ queries $x_v$ with $v \in \Alg$. Thus, we have:
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf)\right] \leq \sum_{v \in \Alg} \Prx_{\boldf \sim \Dno}\left[ x_v \in \bD^q  \right] \mathop{\lsim}^{(\ref{lem:exp-decrease})} 2^q \cdot 1/q! = o(1). 
\end{align*}
{\color{red}I hope the second part of $\calE_1$ follows from the discussion in
  the email thread on March 6.} \blue{Yup, I think this should be fine - it'll follow from the kind of calculations that will be in the proof of \Cref{lem:rad-by-rad}. Shivam and Rocco will fill this in.}
  
  
I think each of the four events follow from a relatively simple union bound. 
For example, for event $\calE_{1,4}$, with a fixed triple of $i,x,z$,
  the probability of the bad event happens over $\bg^i$ is roughly
$$
\frac{1}{N} \cdot 2^{-\text{some big constant}\cdot q}.
$$
This is because we can consider the draw of $\bg^i$ (the relevant part)
  as drawing two standard Gaussians along $x$ and along $y$.
%\end{proof}

We finish the proof by showing that $\calE_{1}$ is implied by the four events together.

\begin{lemma}
$\calE_{1,1}(f)\cap \calE_{1,2}(f)\cap \calE_{1,3}(f)\cap \calE_{1,4}(f)$ implies
  $\calE_{1}(f)$.
\end{lemma}
\begin{proof}
Recall that $Q^q$ denotes the set of $q$ queries made by $\Alg$ when running on $f$.
First $\calE_{1,1}$ implies that the number of nonempty flaps, $i\in [N]$
  with $Q^q\cap F_i\ne \emptyset$, is at most $q^2$.
Fix any nonempty flap $F_i$ and any two points $x,z\in Q^q\cap F_i$.
The case when $x$ and $z$ are colinear is trivial given that $x,z\in \Shell$
  by $\calE_{1,2}$ and thus, $\|x-z\|_2\le 100q$.
  
Consider the case when $x,z$ are non-colinear, with $z=(1+a)x+by$ being
  the decomposition with $x\perp y$, $\|y\|_2=1$ and $b>0$.
Let $\alpha := \|x-z\|_2^2 = a^2+b^2$.    Our goal is to establish that
\begin{equation} \label{eq:goal}
\alpha \leq  250000 q \sqrt{n} .
\end{equation}

We have $\|z\|_2^2 = (1+a)^2 \|x\|_2^2 +  b^2$.
Given that $z\in \Ball(\sqrt{n})$, we have $\|z\|_2\le \sqrt{n}$. So
\[
\|z\|_2^2 = (1+2a)\|x\|_2^2 + \alpha \leq n. 
\]
By $\calE_{1,2}$, we have $x\in \Shell$ and thus, $\|x\|_2\ge \sqrt{n}-100q$.
Plugging it in, we have
\[
(1+2a)(n-200q\sqrt{n}+10000q^2) + \alpha \leq n,
\]
or equivalently,
\begin{equation} \label{eq:a}
\alpha \leq -2an +(1+2a)(200q\sqrt{n}-10000q^2)
\le 200q\sqrt{n}+a(-2n+400q\sqrt{n}-20000q^2). %\le -2cn+200(1+2c)q\sqrt{n}.
%4\sqrt{n} - 2c(n-2\sqrt{n}+1).
\end{equation}
%Since $\alpha \geq 0$ and using $q=o(\sqrt{n})$, we get
%\[
%c \leq {\frac {200q \sqrt{n}}{2n-400q\sqrt{n}+10000q^2}} \leq {\frac {200q} {\sqrt{n}}}.
%\]

Let's consider two cases:

\medskip
\noindent {\bf Case 1:} $a \geq -200q/\sqrt{n}.$  We have from  \Cref{eq:a} (note that
  the coefficient of $a$ is negative and is a value larger than $-2n$) 
%$$2c(n-2\sqrt{n}+1) \geq {\frac {-20}{\sqrt{n}}} \cdot (n-2\sqrt{n}+1) \geq -21\sqrt{n},$$ so \Cref{eq:a} gives
%$
%
$$\alpha \leq 200q\sqrt{n}+2n\cdot \frac{200q}{\sqrt{n}}= 600q\sqrt{n},$$ and we get \Cref{eq:goal}.

\medskip
\noindent {\bf Case 2:} $a < -200q/\sqrt{n}.$  In this case, using $r\le \langle z,g^i\rangle  ,\langle x,g^i\rangle\le r+100q n^{1/4}$ (where the first inequality is because $x,z \in F_i$ and the second is from $\calE_{1,3}$) gives 
\begin{align*}
r &\leq \overbrace{(1+a)\cdot \langle x, g^i\rangle + b \cdot \langle y_i,g^i\rangle}^{=\langle z, g^i\rangle} \leq a\cdot \langle x,g^i\rangle+  \overbrace{{r+100qn^{1/4}}}^{\text{b/c~}\langle x ,g^i\rangle \le r+100q n^{1/4}}  + b\cdot  \overbrace{(100 \sqrt{q})}^{\text{b/c~}|\langle y,g\rangle | \leq 100\sqrt{q}}
%&\leq n^{3/4} - 5n^{1/4} + \sum c_i (100 \log n),
\end{align*}
so (recall that $a<-200q/\sqrt{n}$ is negative and $-a$ is positive)
\[
b\ge \frac{-a\cdot \langle x,g^i\rangle-100qn^{1/4}}{100\sqrt{q}}\ge  \frac{-a r}{200\sqrt{q}}.
\]
%\[
%{\frac {-cn^{3/4}}{200 \log n}} \leq {\frac {-cn^{3/4} - n^{1/4} }{100 \log n}} \leq \sum c_i \text{~(remember, }
%\]
%Now applying Cauchy-Schwarz, we have
%\[
%b\ge 
%\frac{1}{q}\cdot \left({\frac {c^2n^{3/2}}{40000 \log^2 n}}\right)  .
%\]
Recalling that
$\|z\|_2^2=(1+a)^2 \|x\|_2^2 + b^2\le n$ and that $\|x\|_2^2 \geq n-200q\sqrt{n}+10000q^2$, we get
$$
n\ge (1+2a+a^2)(n-200q\sqrt{n})+ {\frac {a^2r^2}{40000 q}} 
\ge (1+2a)(n-200q\sqrt{n})+{\frac {a^2r^2}{40000 q }} 
$$
%\begin{align*}
%& (1+2c+c^2) (n-2\sqrt{n}+1) + \blue{\left({\frac {c^2n^{3/2}}{40000 \log^2 n}}\right)/q'}\\ &\leq 
%(1+2c+c^2) \|x\|^2 + \blue{\left({\frac {c^2n^{3/2}}{40000 \log^2 n}}\right)/q'}\\ &\leq
%(1+2c+c^2) \|x\|^2 + \sum c_i^2 \leq
% n , \text{~and hence}
%\end{align*}
and hence,
\[
a^2 \cdot \frac {r^2}{40000 q}
\leq
200q\sqrt{n} -2a (n-200q\sqrt{n} ).
\]
Recalling that $a<0$, dividing through by $-a$ we get
\[
(-a) \cdot \frac{r^2}{40000q}
\le {\frac {200q\sqrt{n}}{-a}} + 2 (n - 200q\sqrt{n} )
\overbrace{\le }^{\text{~(using $-a\ge 200q/\sqrt{n}$)}}  3n.
\]
So we have
\[
0 <
-a \leq \frac{120000qn}{r^2}.
\]
\red{\rnote{I think we need to bring in the constant hiding in the $r=\Theta(n^{3/4})$ at this point}
Recalling \Cref{eq:a}, we get 
\[
\alpha \leq 200q\sqrt{n} - 2an \leq 200q\sqrt{n} + 240000q\sqrt{n},
\]}
%Now, since $q' \leq n^{0.49}$, we have that
%$\red{INSANITY}= {\frac {n^{3/2}}{40000q' \log^2(n)}} (1 \pm o(1))$, so 
%\[
%Q \leq 4 \sqrt{n} + {\frac {6n^2}{\red{INSANITY}}} 
%\leq 4\sqrt{n} + 240000q\sqrt{n} \log^2(n)(1 \pm o(1))
%\leq 25\sqrt{n} + 250000 q' \sqrt{n} (\log n)^2
%\]
as was to be shown.
\end{proof}

\subsubsection{Proof of Lemma~\ref{lem:ev3}}

%\enote{I'm hopeful this lemma will be straight-forward given the events. Essentially, we just need to ``randomize'' with respect to the action subspaces and perform union bounds only with respect to $q$.}

For $\overline{\calE_2(f)}\cap \calE_1(f)$ to happen, there must exist a level
  $k\in [q]$ such that
\begin{flushleft}\begin{itemize}
\item After the the first $k-1$ queries $Q=Q^{k-1}$, $\calE_1(f)$ holds, i.e., the number of
  flaps $F_i$ with $Q \cap F_i\ne\emptyset$ is at most $q^2$. In every such $F_i$, every two points in $Q \cap F_i$ have distance at most
  $500 \sqrt{q}n^{1/4}$ and share the same value of 
  $$
  \Indicator\sbra{\langle v^i ,x \rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]},
  $$
  which we denote by $b_i\in \{0,1\}$.
\item Let $y$ be the $k$-th query.
There exists an $i$ such that $Q\cap F_i\ne \emptyset$ and $y\in F_i$ such that  
\begin{equation}\label{hehe1}
\|y-x\|\le 500 \sqrt{q}n^{1/4}
\end{equation}
for all $x\in Q\cap F_i$ (the number of such $i$ is at most $q$) but
$$
\Indicator\sbra{\langle v^i ,x \rangle \notin [-\sqrt{n}/2,\sqrt{n}/2]}\ne b_i.
$$
\end{itemize}\end{flushleft}

We prove below that when $q\ll ?$, the probability of the event above 
  for a fixed $k$ is $o(1/q)$ and thus, Lemma~\ref{lem:ev3} follows by applying a union bound on $k$.
This follows from a union bound on all $i\in [N]$ such that 
  $Q\cap F_i\ne \emptyset$ and every $x\in Q\cap F_i$ satisfies (\ref{hehe1}), taking $X$ (or $z$) below as $Q\cap F_i$ (or $y$, respectively)
  projected on the space orthogonal to $g^i$
  and $b$ as $b_i$.
Formally the $n$ in the lemma below should also be set to be $n-1$.
%This follows from a union bound on the event of $y\in all $i\in [N]$ with $Q\cap F_i\ne \emptyset$ 

\begin{lemma}
Let $b\in \{0,1\}$, and
let $X$ be a set of at most $q$ points in $\Ball(\sqrt{n})$ and $y\in \Ball(\sqrt{n})$
  such that~every pair of points in $X\cup \{y\}$ have
  distance at most $500\sqrt{q}n^{1/4}$.
Then over the draw~of $\bv\sim N(0,I_n)$, the probability of
  $\Indicator[\langle  \bv,y\rangle \notin[-\sqrt{n}/2,\sqrt{n}/2]]\ne b$ conditioning on the event that
  $\Indicator[\langle \bv,x\rangle \notin[-\sqrt{n}/2,\sqrt{n}/2]]=b$ for all $x\in X$ is at most $O(\sqrt{q} \log n/n^{1/4})$.
\end{lemma}
\begin{proof}
Fix a point $x^*\in X$. We show that (1) the probability of $\Indicator[\langle \bv,x\rangle \notin[-\sqrt{n}/2,\sqrt{n}/2]]=b$
  for all $x$ is at least $\Omega(1)$; and (2) the probability of 
$$
\Indicator[\langle  \bv,y\rangle \notin[-\sqrt{n}/2,\sqrt{n}/2]]\ne \Indicator[\langle  \bv,x^*\rangle \notin[-\sqrt{n}/2,\sqrt{n}/2]]
$$
is at most $???$. The lemma then follows.

To analyze (1), we first note that the probability of $\langle \bv, x^*\rangle$ lying in  the union of
$$
[-\sqrt{n}/2-50000 \sqrt{q}n^{1/4}\log n,-\sqrt{n}+50000\sqrt{q}n^{1/4}\log n]$$
and 
$$
[ \sqrt{n}/2-50000 \sqrt{q}n^{1/4}\log n, \sqrt{n}+50000\sqrt{q}n^{1/4}\log n]
$$
is at most $O(\sqrt{q}\log n/n^{1/4})$.\xnote{This is just calculation using $\|x^*\|=\sqrt{n}$.
I think this is about the worst case but maybe we should justify.}
On the other hand, given that $\|x-x^*\|\le 500\sqrt{q}n^{1/4}$,
  it follows from a union bound $x\in X$ that 
$$
\left|\langle\bv,x-x^*\rangle\right|> 100000\sqrt{q}n^{1/4}\log n
$$
for some $x\in X$
with probability at most $o(1)$.
Given that (1) happens when the two events above do not occur, we have that (1) holds with probability at least $\Omega(1)$.

The analysis of (2) is similar. 
(2) happens when either $\langle \bv,x^*\rangle$  lies the union of  () and ()
  or $\langle \bv, y-x^*\rangle$ satisfies the same inequality ().
So  (2) happens with probability at most $O(\sqrt{q}\log n/n^{1/4})$.
\end{proof}
%Skethc: Fix $g^1,\ldots,g^N$ that satisfy $\calE_1$. 
%Then apply union bound on $v^i$ with a nonempty $Q^q$
%\subsubsection{Proof of Lemma~\ref{lem:ev2}}

%Given a set of queries $Q$ made by $\Alg$ such as $Q^k$ for some $k\le q$,
%  we say a nonempty, regular flap $F_i$ is \emph{nice} with respect to $Q$ 
%  if the following condition holds:
%\begin{flushleft}\begin{itemize}
%%\item $Q\cap F_i\subset \Shell$;
%\item Let $x\in Q$ be the query point that discovers $F_i$.
%  There exist $\ell$ unit vectors $y_1,\ldots,y_\ell$ for some $\ell<|Q\cap F_i|$
%  such that $x,y_1,\ldots,y_\ell$ form an orthogonal basis, $|\langle g^i,y_j\rangle|\le %100\log n$ for all $j\in [\ell]$, and $Q\cap F_i\subset \Span(x,y_1,\ldots,y_\ell)$.
%\end{itemize}\end{flushleft}
%Notice that when $F_i$ is just discovered by a query point $x$,
%  $Q\cap F_i$ is trivially nice by taking $\ell=0$ (unless $x\notin \Shell$ or $\langle %g^i,x\rangle>r+100q n^{1/4}$
%  in which case $Q\cap F_i$ is not regular).
%  
%The proof of Lemma \ref{lem:ev2} consists of two steps. 
%In Lemma \ref{lem:sufficient} we show that a sufficient condition for $%\overline{\calE_2(f)}$ is that 
%  at the end of the execution of $\Alg$ on $f$, for any of the first $q^2$ nonempty flaps %$F_i$
%  with respect to $Q^q$, $F_i$ being regular implies that it is nice.
%%  the first $q^2$ flaps $F_i$ with $\emptyset\ne Q^q\cap F_i\subset \Shell$ are all nice.
%In Lemma \ref{lem:prob}, we show that the latter happens with probability at least $1-%o(1)$.
%%We start with the following equivalent description of event $\calE_2(f)$:%

%\begin{lemma}\label{lem:sufficient}
%Let $f$ be a function in the support of $\Dno$ and $Q^q$ be the points queried
%  by $\Alg$ when executing on $f$.
%Then $\overline{\calE_2(f)}$ holds if for every of the first $q^2$ nonempty flaps $F_i$
%%  with respect to $Q^q$, $F_i$ being regular implies that it is nice. %flaps $F_i$ are all nice.
%\end{lemma}
%\begin{proof}
%%Let $F_i$ be one of the first $q^2$ nonempty flaps that is both regular and nice.
%We show that every two points in $Q^q\cap F_i$ have
%  distance at most $1000 q n^{1/4} \log n .$  
%To this end, letting $x$ be the query in $Q^q$ that discovers $F_i$,
%  it suffices to show that $\|x-z\|_2\le 500 q n^{1/4} \log n $ for every $z\in Q^q\cap %F_i$.
  
%Since $F_i$ is nice, we write $y_1,\ldots,y_\ell$, for some $\ell< |Q^q\cap F_i|\le q$,
%  to denote the unit vectors as in the definition of $F_i$ being nice.
%Let $z$ be any point in $Q^q\cap F_i$. 
%We show below that 
%$$
%\|x-z\|_2^2\le 250000 q^2\sqrt{n} \log^2 n.
%$$
%Given that $z\in Q^q\cap F_i\subset \conv(x,y_1,\ldots,y_\ell)$,
%  we can write $z$ uniquely as $$z=x + cx + c_1 y_1 + \cdots + c_{\ell} y_{\ell}.$$
%Let $\alpha := \|x-z\|_2^2 = c^2 \|x\|_2^2 + \sum_{i=1}^\ell c_i^2.$    Our goal is to %establish that\xnote{Some notational conflict: We should use $\sum_{j}$ instead of $%\sum_i$; some $g$ below should be $g^i$.}
%\begin{equation} \label{eq:goal}
%\alpha \leq  250000 q \sqrt{n} \log^2 n .
%\end{equation}

%We have $\|z\|_2^2 = (1+c)^2 \|x\|_2^2 +  \sum_{i=1}^{\ell} c_i^2$.
%Given that $z\in \Ball(\sqrt{n})$, we have $\|z\|_2\le \sqrt{n}$. So
%\[
%\|z\|_2^2 = (1+2c)\|x\|_2^2 + \alpha \leq n. 
%\]
%Given that $F_i$ is regular, we have $x\in \Shell$ and thus, $\|x\|_2\ge \sqrt{n}-100q$.
%Plugging it in, we have
%\[
%(1+2c)(n-200q\sqrt{n}+10000q^2) + \alpha \leq n,
%\]
%or equivalently,
%\begin{equation} \label{eq:a}
%\alpha \leq -2cn +(1+2c)(200q\sqrt{n}-10000q^2)
%\le 200q\sqrt{n}+c(-2n+400q\sqrt{n}-20000q^2). %\le -2cn+200(1+2c)q\sqrt{n}.
%5%4\sqrt{n} - 2c(n-2\sqrt{n}+1).
%5\end{equation}
%%Since $\alpha \geq 0$ and using $q=o(\sqrt{n})$, we get
%%\[
%%c \leq {\frac {200q \sqrt{n}}{2n-400q\sqrt{n}+10000q^2}} \leq {\frac {200q} {\sqrt{n}}}.
%%\]%

%Let's consider two cases:

%\medskip
%\noindent {\bf Case 1:} $c \geq -200q/\sqrt{n}.$  We have from  \Cref{eq:a} (note that
%  the coefficient of $c$ is negative) 
%$$2c(n-2\sqrt{n}+1) \geq {\frac {-20}{\sqrt{n}}} \cdot (n-2\sqrt{n}+1) \geq -21\sqrt{n},$$ so \Cref{eq:a} gives
%$
%
%$$\alpha \leq 200q\sqrt{n}+2n\cdot \frac{200q}{\sqrt{n}}= 600q\sqrt{n},$$ and we get %\Cref{eq:goal}.

%\medskip
%\noindent {\bf Case 2:} $c < -200q/\sqrt{n}.$  In this case, the fact that $n^{3/4}\le %\langle z,g^i\rangle  ,\langle x,g^i\rangle\le n^{3/4}+100q n^{1/4}$ gives %
%\begin{align*}
%n^{3/4} &\leq \overbrace{(1+c)\langle x, g\rangle + \sum_{i=1}^{\ell} c_i \langle %y_i,g\rangle}^{=z \cdot g} \leq c\langle x,g\rangle+  \overbrace{{n^{3/4}+100qn^{1/4}}}^{\text{b/c~}g \cdot x \leq n^{3/4}}  + \sum_{i=1}^\ell |c_i| \overbrace{(100 \log n)}^{\text{b/c~}|g \cdot y^i| \leq 100 \log n}
%&\leq n^{3/4} - 5n^{1/4} + \sum c_i (100 \log n),
%\end{align*}
%so (recall that $c<-200q/\sqrt{n}$ is negative and $-c$ is positive)
%\[
%\sum_{i=1}^\ell |c_i|\ge \frac{-c\langle x,g\rangle-100qn^{1/4}}{100\log n}\ge  \frac{-c %n^{3/4}}{200\log n}.
%\]
%\[
%{\frac {-cn^{3/4}}{200 \log n}} \leq {\frac {-cn^{3/4} - n^{1/4} }{100 \log n}} \leq \sum c_i \text{~(remember, }
%\]
%Now applying Cauchy-Schwarz, we have
%\[
%\sum_{i=1}^\ell c_i^2\ge 
%\frac{1}{q}\cdot \left({\frac {c^2n^{3/2}}{40000 \log^2 n}}\right)  .
%\]
%Recalling that
%$\|z\|_2^2=(1+c)^2 \|x\|_2^2 + \sum_{i=1}^\ell c_i^2 \leq n$ and that $\|x\|_2^2 \geq %n-200q\sqrt{n}+10000q^2$, we get
%$$
%n\ge (1+2c+c^2)(n-200q\sqrt{n})+ {\frac {c^2n^{3/2}}{40000 q\log^2 n}} 
%\ge (1+2c)(n-200q\sqrt{n})+{\frac {c^2n^{3/2}}{40000 q\log^2 n}} 
%$$
%\begin{align*}
%& (1+2c+c^2) (n-2\sqrt{n}+1) + \blue{\left({\frac {c^2n^{3/2}}{40000 \log^2 n}}\right)/q'}\\ &\leq 
%(1+2c+c^2) \|x\|^2 + \blue{\left({\frac {c^2n^{3/2}}{40000 \log^2 n}}\right)/q'}\\ &\leq
%(1+2c+c^2) \|x\|^2 + \sum c_i^2 \leq
% n , \text{~and hence}
%\end{align*}
%and hence,
%\[
%c^2 \cdot \frac {n^{3/2}}{40000 q\log^2n}
%\leq
%200q\sqrt{n} -2c (n-200q\sqrt{n} ).
%\]
%Recalling that $c<0$, dividing through by $-c$ we get
%\[
%(-c) \cdot \frac{n^{3/2}}{40000q\log^2n}
%\le {\frac {200q\sqrt{n}}{-c}} + 2 (n - 200q\sqrt{n} )
%\overbrace{\le }^{\text{~(using $-c\ge 200q/\sqrt{n}$)}}  3n.
%\]
%So we have
%\[
%0 <
%-c \leq \frac{120000q \log^2 n}{\sqrt{n}}.
%\]
%Recalling \Cref{eq:a}, we get 
%\[
%\alpha \leq 200q\sqrt{n} - 2cn \leq 200q\sqrt{n} + 120000q\sqrt{n}\log^2 n,
%\]
%Now, since $q' \leq n^{0.49}$, we have that
%$\red{INSANITY}= {\frac {n^{3/2}}{40000q' \log^2(n)}} (1 \pm o(1))$, so 
%\[
%Q \leq 4 \sqrt{n} + {\frac {6n^2}{\red{INSANITY}}} 
%\leq 4\sqrt{n} + 240000q\sqrt{n} \log^2(n)(1 \pm o(1))
%\leq 25\sqrt{n} + 250000 q' \sqrt{n} (\log n)^2
%\]
%as was to be shown.
%\end{proof}


%Let $\calE_2'(f)$ denote the event that at the end of execution of $\Alg$ on $f$,
%%  at least one of the first $q^2$ nonempty flaps $F_i$ satisfies
%  $F_i$ is regular but not nice.

%\begin{lemma}\label{lem:prob}
%The event $\calE_2'(f)$ happens with probability $o(1)$ as $\boldf\sim \Dno$.
%\end{lemma}
%\begin{proof}
%For $\calE_2'$ to happen, there must be a $k\le q$ such that
%\begin{flushleft}\begin{itemize}
%\item With respect to $Q^k$, for every of the first $q^2$ nonempty flaps $F_i$,
%  $F_i$ being regular implies that $F_i$ is nice.
%  Let $I$ denote the set of the first $q^2$ nonempty flaps that are regular (and nice).
%\item Let $x$ be the next query point satisfying $x\in \Shell$. 
%  There exists an $i\in I$ such that $x\notin \Span(Q^k\cap F_i)$ and $|\langle %y,g^i\rangle|>100\log n$,
%  where $y$ is the unit vector that is the component of $x$ that is orthogonal to $%\Span(Q^k\cap F_i)$%.
%\end{itemize}\end{flushleft}
%This happens with probability $o(1)$ by a union bound on $k$ and $I$.
%\end{proof}


%\enote{I think this one will be the more complicated argument.}



==> sections/one-sided-adaptive.tex <==
%!TEX root = ../ctlb.tex

\newpage

\section{One-sided adaptive lower bound}
\label{sec:one-sided-adaptive}

\begin{theorem} [One-sided adaptive lower bound, restated] \label{thm:one-sided2}
For some absolute constant $\eps>0$, any one-sided $\eps$-tester for convexity  over $N(0,I_n)$ (which may be adaptive) must use $n^{\Omega(1)}$ queries.
\end{theorem}

At a high level, the proof of \Cref{thm:one-sided} works by (1) first defining a distribution $\Dno$ of ``no-functions'' (Boolean-valued functions over $\R^n$, or equivalently, subsets of $\R^n$), and showing that an $\Omega(1)$ fraction of draws from $\Dno$ yield sets which are $\Omega(1)$-far from convex; and (2) then arguing that for a suitable absolute constant $c>0$, any $n^c$-query algorithm (even an adaptive one) has only an $o(1)$ probability of querying a set of points whose labels are inconsistent with every convex set in $\R^n$.
In the next subsection we describe the distribution $\Dno$.
 
\subsection{The distribution $\Dno$ of far-from-convex sets}

\subsubsection{Setup}

First some useful notation and terminology:  we define the \emph{shell} to be the set $\Shell \subset \R^n,$
\begin{equation} \label{eq:shell}
\Shell := \cbra{x \in \R^n \ : \ \|x\| \in [\sqrt{n}-1,\sqrt{n}+1]}.
\end{equation}
We will see that every function $f \in \Dno$ outputs 1 on every input $x$ with $\|x\| < \sqrt{n}-1$ and outputs 1 on every input $x$ with $\|x\| > \sqrt{n}+1$.  To describe how functions in $\Dno$ behave on inputs in $\Shell$, we require some more setup.

\medskip
\noindent {\bf Nazarov's body.}
Fix $N:= 2^{\sqrt{n}}$ (we assume without loss of generality that $n$ is a perfect square, so $N$ is an integer).
For each $i\in[N]$, draw $\bg^i = (\bg^i_1,\dots,\bg^i_n) \sim N(0,I_n)$. Let $\bH_i$ denote the  halfspace 
\begin{equation}
\bH_i := \cbra{x\in\R^n \ : \ \abra{x, \bg^i} \leq r} \label{eq:boldH}
\end{equation}
(we will specify $r$ below).  
Let 
\begin{equation}
\label{eq:B}
\bB = \bH_1 \cap \cdots \cap \bH_N \subset \R^{n};
\end{equation} we refer to $\bB$ as the ``Nazarov body,''
and we write ``$\bB \sim \mathrm{Naz}(r,N)$'' to indicate that $\bB$ is a random body constructed in this way.
We choose $r$ to be the unique value such that for any point $x \in \R^n$ with $\|x\|=\sqrt{n}$ (we may take $x=(\sqrt{n},0,\dots,0)$ for concreteness; note that all points at distance $\sqrt{n}$ are equivalent, by the rotational symmetry of the $N(0,I_n)$ distribution), we have 
$\Pr_{\bB \sim \mathrm{Naz}(r,N)}[x \in \bB]=1/2.$  (We will argue later that $r \approx n^{3/4}.$)


For each $i \in [N]$ we will also consider the halfspace $\bH'_i$ obtained by moving the defining hyperplane slightly in towards the origin:
\[
\bH'_i := \cbra{x\in\R^{n+1} : \abra{x, \bg^i} \leq  r - c_1 n^{1/4}},
\]
where $c_1>0$ is an absolute constant that will be specified later.
For $i \in [N]$ we define the set $\bB_i$ ($\bB_i$ is for ``{\bf b}oundary region of facet $i$'') to be the set of points in $\bB$ which are falsified by $\bH'_i$, i.e.
\[
\bB_i = \bB \setminus \bH'_i
\]
(in Figure~1 this is the red $\bF_i$ region plus its two adjacent blue diamonds).
We also define $\bS_i$ to be the infinite ``$i$-th {\bf s}lab''
\[
\bS_i := \bH_i \setminus \bH'_i = \cbra{x \in \R^n \ : r - c_1 n^{1/4} < \abra{x, \bg^i} \leq r},
\] 
so we have $\bB_i = \bB \cap \bS_i$.
We define the set $\bF_i$ (for ``{\bf f}lap'') to be the points in $\bB$ which are falsified by a unique $\bH'_i$, i.e.,
\[
\bF_i = \{x \in \bB: x \notin \bH'_i \text{~and for all~}j \neq i, j \in [N],  \text{~we have~}x \in \bH'_j\}.
\]

\begin{figure} \label{fig:nazzy}
 \begin{center}
\includegraphics[width=0.7\textwidth]{a}
\end{center}
\caption{The Nazarov body.}
\end{figure}

The regions $\bF_i$ and $\bF_j$ are shaded red in Figure~1. 
We define 
\begin{equation} \label{eq:F}
\bF := \bF_1 \sqcup \cdots \sqcup \bF_N
\end{equation}
(note that the $\bF_i$'s are disjoint), and we define 
\begin{equation} \label{eq:Bprime}
\bB' := \bH'_1 \cap \cdots \cap \bH'_N.
\end{equation} 
We will sometimes refer to $\bB'$ as the ``contracted Nazarov body''. 

For $T \subseteq [N]$, we define $\bD_T$ to be the points of $\bB$ which are falsified by exactly those $\bH'_j$'s for which $j$ belongs to $T$, i.e.
\begin{equation} \label{eq:DT}
\bD_T = \cbra{x \in \bB \ : \text{~for $j \in T$ we have~}
x \notin \bH'_j \text{~and for $j \in [N]\setminus T$ we have~}x \in \bH'_j
 }.
 \end{equation}
Note that $\bD_{\{j\}}$ is another name for $\bF_j$, that $\bD_{\emptyset}$ is another name for $\bB'$, and that $\bB_i = \cup_{T \ni i} \bD_T$.
We define $\bD$ (for ``{\bf d}og ear'') to be the union of the $\bD_T$'s over all sets $T$ of size at least two:
\begin{equation} \label{eq:D}
\bD := \bigcup_{|T| \geq 2, T \subseteq N} \bD_T.
\end{equation}
For $i \in [N]$, we further define
\begin{equation} \label{eq:Dsuperi}
\bD^i = \bigsqcup_{T \subset N, |T|=i} \bD_T
\end{equation}
to be the disjoint union of the $\bD_T$'s across all $T$ of size exactly $i$.

\medskip
\noindent {\bf The ``action directions.''} 
For each $i \in [N]$, draw a random Gaussian vector $\bv^i =(\bv^i_1,\dots,\bv^i_n) \sim N(0,I_n)$ (independent of everything else).  We say that $\bv^i$ is the \emph{action direction} for the $i$-th halfspace.

%Let's also define the 1-dimensional interval
%\[
%I := \sbra{-1/2, 1/2} \subset \R
%\]
%since we will need it soon.

\subsection{The distribution $\Dno$}

For a fixed setting of $\vec{H} := (H_1,\dots,H_N)$ (which also specifies $H'_1,\dots,H'_N$ and hence the $S_i$'s, $F_i$'s, $D_T$'s, $D$, $B$, and $B'$) and a fixed setting of $\vec{v}:=(v^1,\dots,v^N)$, we define the function $g_{\vec{H},\vec{v}}: \R^n \to \{0,1\}$ as follows:
 
 %\rnote{Minor thing: in the previous version we had been saying, in the first line of the definition of $g_{C,\vec{H},P}$, that $g_{C,\vec{H},P}(x)$ is 0 if $\|x\|$ (not $\|x_C\|$) is outside the right range. But I think this is a little inconsistent with e.g. the second line in the definition of $g_{C,\vec{H},P}(x)$ --- it's possible for $\|x\|$ to be larger than $\sqrt{n}+10\sqrt{\ln(1/\eps)}$ but for $x$ to also lie in $B'$, if, e.g., $x$ had a freakishly large component $x_A$ (recall that $B'$ is defined only in terms of what happens in the control space, i.e. in terms of $x_C$).}

\[
g_{\vec{H},\vec{v}}(x) = \begin{cases}
0 & \text{if~} x \notin B ;\\
1 & \text{if~} x \in B' \text{~(equivalently, $x \in D_{\emptyset}$)};\\
\bigwedge_{j \in T}\Indicator\sbra{v^j \cdot x \notin [-1/2,1/2]} & \text{if~} x \in D_T
\text{~for some~}\emptyset \neq T \subseteq [N].
\end{cases}
\]

A random function $\boldf \sim \Dno$ is drawn as follows:  we draw $\vec{\bH}$ as in \Cref{eq:boldH},  we draw $\vec{\bv}$ by independently choosing each $\bv^i \sim N(0,I_n)$, and we set

\[
\boldf_{\vec{H},\vec{v}}(x) = \begin{cases}
0 & \text{if~} \|x\| > \sqrt{n}+1 ;\\
1 & \text{if~} \|x\| < \sqrt{n}-1 ;\\
\bg_{\vec{\bH},\vec{\bv}}(x) & \text{if~} \|x\| \in \Shell.
\end{cases}
\]





\subsection{Useful properties of the $\Dno$-sets}

We will require the following lemma, which states that the expected volume of $\bD^i$ decreases very rapidly as a function of $i$:

\blue{
\begin{lemma}[Erik says maybe the following is good enough for the one-sided adaptive part] 
\label{lem:rad-by-rad}
Fix any radius $r$ we need to worry about, in $[\sqrt{n}-1,\sqrt{n}+1]$, and fix a point $z$ with $\|z\|_2=r$.  Fix $q=n^c$ for a small constant $c$.  Then for a random Nazarov body, we have $\Pr[z \in \sqcup_{i \geq q}\bD^i] \leq O(1/q!).$  (Even a RHS of $1/4^q$ would suffice for us; this will fight a union bound over all $(1.0\cdot 2)^q$ leaves of the tree.)
\end{lemma}
}

%\begin{lemma} \label{lem:exp-decrease}
%\red{Let $m = \green{\log n}.$ For $1 \leq i \leq m$, we have
%$\sum_{j \geq i} \Ex_{\boldf \sim \Dno}[\Vol(\bD^j)] \leq O(1/i!) + 1/n$.}
%\rnote{Is this what we need? For the tolerant construction, I think we needed that $\Vol(\bD^1)$ dominates $\sum_{j\geq 2} \Vol(\bD^j)$.}


%
%Also, I think we might additionally need the statement to give us that
%$\Ex_{\boldf}[\Vol(\cup_{i \in [m+1,N]} \bD^i)]$ is not too large.}
%\end{lemma}

\red{(Mostly ignore the following since we plan to analyze the $\bD^i$'s instead of the $\bD'^i$'s)}

We provide some setup for this lemma before entering into the proof.
For $T \subseteq [N]$ define 
\[
\bD'_T := \cbra{x \in \R^n \ : \text{for each~}i \in [N], x 
\in \bS_i \text{~iff~}i \in T
},
\]
i.e.~the set of points in $\R^n$ that belong to precisely the slabs indexed by the elements of $T$.
For $T \subseteq [N]$ define 
\[
\bD'^i = \bigsqcup_{T \subset N, |T|=i} \bD'_T
\]
Note that $\bD_T=\bB \cap \bD'_T$ and $\bD'^i = \bB \cap \bD^i$.
%Hence \Cref{lem:exp-decrease} is an immediate corollary of the following:
%\begin{lemma} \label{lem:exp-decrease2}
%\red{Let $m = \green{\log n}.$ For $1 \leq i \leq m$, we have
%$\sum_{j \geq i} \Ex_{\boldf \sim \Dno}[\Vol(\bD^j)] \leq O(1/i!) + 1/n$.}
%\end{lemma}

The main idea behind \Cref{lem:exp-decrease2} is to perform the analysis on a ``radius-by-radius'' basis.
For any $t>0$, define $p_t \in [0,1]$ to be the value such that every $x \in \R^n$ with $\|x\|_2=t$ has $\Pr[x \in \bS_1]=p_t$ (this value will be the same for all $x$ with $\|x\|_2=t$ by rotational symmetry of $N(0,I_n)$).
It follows that
\begin{equation}
\label{eq:fixed-radius-t}
\text{ for $\|x\|_2=t,$ we have~}
\Pr[x \in \bD'_T]=p_t^{|T|} \cdot (1-p_t)^{N-|T|}.
\end{equation}
Let us analyze this quantity:


\bigskip\bigskip\bigskip\bigskip

\blue{create some BLAHBLAH statement roughly along the lines of the analysis in \href{https://docs.google.com/document/d/1Z45IzhgP4Ke-Y_1ZtTOfkXJ7Ewg6mR5fTJumIUtYxeI/edit}{this Google Drive file}, establishing that for any $z$ with $\|z\| = \sqrt{n}+\Delta$, where $|\Delta| \leq$ (something), we have $\Pr_{\boldf \sim \Dno}[z \in \bD'^i] = such-and-such$.  Using the fact that the variance of the $\chi^2(n)$ distribution is $2n$, we need to work out what the (something) needs to be so that we can combine the radius-by-radius bounds and only incur a small acceptable error because of outcomes of $\|\bg\|_2$ which come out outside of $[\sqrt{n}-\Delta,\sqrt{n}+\Delta]$).}

\bigskip\bigskip\bigskip\bigskip
 
With \blue{BLAHBLAH} in hand, we can bound the volume of $\bD'^i$ as follows. 
Recalling \Cref{eq:fixed-radius-t}, we have
\[
\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)]=
{N \choose i} \cdot \Ex_{\bt \sim \chi(n)}\sbra{ p_{\bt}^{i} \cdot (1-p_{\bt})^{N-i}}.
\]


\bigskip \bigskip \bigskip \bigskip \bigskip \bigskip \bigskip \bigskip 

\blue{
\subsubsection{High-order $\bD_T$'s have small volume}

\medskip

We think we will need a lemma like the following:
\begin{lemma} \label{lem:exp-decrease-old}
$\Ex_{\boldf \sim \Dno}[\Vol(\bD^i)] \leq 2^{-\Omega(i)}.$
\end{lemma}

\noindent
\emph{Proof sketch for \Cref{lem:exp-decrease}.}
We observe that $\bD_T \subseteq \bD'_T$. 
%(To see this, consider any $x \in \bD_T$. We have $x \in \bB$ so $x \in \bH_i$ for all $i \in [N]$, and $x \in \bH'_i$ for exactly those $i \in [N]$ that do not belong to $T$. Hence $x \in \bS_i$ for exactly those $i \in [N]$ that belong to $T$, so $x \in \bD'_T.$)
So to show that $\Ex_{\boldf \sim \Dno}[\Vol(\bD_i)] \leq 2^{-\Omega(i)},$ it suffices to show that $\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)] \leq 2^{-\Omega(i)}.$ 

%Recall that for $i \in [N]$ we have that slab $i$ is
%\[
%\bS_i = \bH_i \setminus \bH'_i
%\]
%(so $\bB_i \subseteq \bS_i$ because $\bS_i$, unlike $\bB_i$, may contain points that are outside of $\bB$). 


We argue that $\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)] \leq 2^{-\Omega(i)}$ by arguing radius-by-radius.  Given a real value $t > 0$, any $x \in \R^n$ with $\|x\|_2=t$ has $\Pr[x \in \bS_1]=p_t$ where $p_t = \red{BLAH}$ and hence
$\Pr[x \in \bD'_T]=p_t^{|T|} \cdot (1-p_t)^{N-|T|}$, so 
\[
\Ex_{\boldf \sim \Dno}[\Vol(\bD'^i)]=
{N \choose i} \cdot \Avg_{\bt \sim \chi(n)}\sbra{ p_{\bt}^{i} \cdot (1-p_{\bt})^{N-i}}
\]
See \href{https://docs.google.com/document/d/1Z45IzhgP4Ke-Y_1ZtTOfkXJ7Ewg6mR5fTJumIUtYxeI/edit}{this Google Drive file} for a sketch of how to prove the radius-by-radius statement or \Cref{lem:exp-decrease}.

\qed

}

\subsection{Sets in $\Dno$ are far from convex}

\blue{
We need a constant fraction of the no-functions to be constant-far from convex:
\begin{claim} 
With probability $\Omega(1)$ over a draw of $\boldf \sim \Dno$, we have that $\boldf$ is $\Omega(1)$-far from every convex set in $\R^n$ (w.r.t. Gaussian volume).
\end{claim}
\noindent \emph{Sketch of justification:} This follows from having $\Ex_{\boldf \sim \Dno}\sbra{\dist(\boldf,\mathrm{convex})}=\Omega(1).$ The idea for why $\Ex_{\boldf \sim \Dno}\sbra{\dist(\boldf,\mathrm{convex})}=\Omega(1)$ is roughly because (i) $\Ex_{\bH}\sbra{\Vol(\bF)}=\Omega(1)$ (this is something we will argue in the tolerant non-adaptive lower bound construction), (ii) $\Vol[\bF]=\sum_{i \in [N]}\Vol[\bF_i]$, and (iii) for a given flap $\bF_i$ we should have that (since $\bv^i$ is almost orthogonal to the direction $\bg^i$ of the hyperplane $\bH_i$ defining $\bF_i$) we can get violating triples (three points in a line segment, where the middle point is labeled 0 and the two outer points are labeled 1, and the line segment is in the direction of $\bv^i$) that in expectation cover a constant fraction of the Gaussian volume of $\bF_i$.  (This needs to be worked out in more detail but we think it should be okay.)
% $\Ex[\Vol(\bF_i \cap \{x: |\abra{\bv^i,x}| \in [-0.5,0.5]\}] \geq \Omega(1) \cdot \Ex[\Vol(\bF_i)]$. This last property should let us argue ``line segment by line segment'' to get violating triples:  fix a segment in $\bF_i$ by specifying everything but the projection in direction $v^i$, so points on the segment vary only in their value of $\abra{x,\bv^i}.$ If there 
\qed
}
\subsection{Proof of \Cref{thm:one-sided}}

\newcommand{\Alg}{\mathrm{Alg}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\lsim}{\lesssim}
\newcommand{\conv}{\mathrm{conv}}

\enote{I started going through the main structure of the argument and diving up into some lemmas. I may be mistaken on the specific events that we need, and we can hopefully discuss these on our Tuesday meeting. }

\begin{definition}[Adaptive Algorithms as Binary Trees]
Fix $n, q \in \N$. A $q$-query deterministic algorithm, $\Alg$, for testing convexity in $\R^n$ is specified by a rooted binary tree of depth $q$ where each node contains the following information:
\begin{itemize}
\item Each node $v$ which is a not a leaf contains a query vector $x_v \in \R^n$, as well as two out-going edges, one labeled 0 and one labeled 1, to nodes which we label $v(0)$ and $v(1)$, respectively.
\item Each leaf node $v$ contains an output $o_v$ which is set to \emph{``accept''} or \emph{``reject.''} 
\end{itemize}
By adding nodes which repeat the queries, we may assume, without loss of generality, that the depth of every leaf of the tree is exactly $q$. Furthermore, we may assume without loss of generality that every $x_v$ {\color{red}satisfies $\|x_v\|_2\le \sqrt{n}+1$}\xnote{As we discussed in the email, ALG should be allowed to query points
  $x_v$ with $\|x_v\|_2<\sqrt{n}-1$.}. \blue{This is because every point $y$ with $\|y\| > \sqrt{n}+1$ must have $f(y)=0$ for every function $f$ in the support of $\Dno$, and hence such a point $y$ cannot participate in a collection of labeled points which witness that such an $f$ is not convex (i.e.~a collection of points $x_1,\dots, x_{\ell}, y$ with $y \in \conv(x_1,\dots, x_{\ell})$, $f(y) = 0$ and $f(x_1) = \dots = f(x_{\ell}) = 1$). (Note that even though every point $x$ with $\|x\| <\sqrt{n}-1$ must have $f(x)=1$ for every $f$ in the support of $\Dno$, it may still be useful for a one-sided tester to query such points, since they can be used in constructing a witness of the $f$ non-convexity of $f$.)}\rnote{Since this point was subtle enough to escape us before Xi noticed it, I added a quick mention for the reader.)}
  
  
\end{definition}
A $q$-query deterministic algorithm $\Alg$ executes on a function $f \colon \R^n \to \{0,1\}$ by taking the natural root-to-leaf path given by following the function values which the oracle returns at the queries within each of the nodes. In particular, we will make repeated use of the following definitions which capture the execution of the algorithm $\Alg$ on a function $f$:
\begin{itemize}
\item The node $v^0$ is the root of the tree, which is the starting point of the root-to-leaf path. Then, the nodes $v^1,\dots, v^q$ indicate the root-to-leaf path generated by executing the algorithm on the function $f$. In particular, at time step $t \in \{ 0, \dots, q-1\}$, we have $v^{t+1} = v^{t}(f(x_{v^{t}}))$
\item The set $Q^0$ is defined to be $\emptyset$, and for $t \in \{0, \dots, q-1\}$ the set $Q^{t+1}$ is defined to be $Q^{t} \cup \{ x_{v^{t}} \} \subset \R^n$.
Thus $Q^{t+1}$ is the set of vectors that are queried at time steps prior to $t+1$.
\end{itemize}
Once the algorithm reaches the leaf node $v^{q}$, the algorithm outputs $o_{v^q}$, and we will refer to $\Alg(f)$ as the output (``accept'' or ``reject'') produced by the algorithm. It is trivial to see that since any $q$-query deterministic algorithm corresponds to a tree of depth $q$, the total number of query vectors $x_v \in \R^n$ across all nodes of the tree is at most $2^q$. Our goal is to show that, if $\Alg$ is a $q$-query deterministic algorithm which makes \emph{one-sided error}, then
\begin{align}
\Prx_{\boldf \sim \Dno}\left[ \Alg(\boldf) = \text{``reject''}\right] = o(1).  \label{eq:adapt-final-exp}
\end{align}
Recall that implicit in a draw of $\boldf \sim \Dno$ are vectors $\bg^1,\dots, \bg^{N} \in \R^n$ and $\bv^1,\dots,\bv^{N} \in \R^n$, and that the vectors $\bg^1,\dots,\bg^N$ define $\bH_i$, $\bH'_i$, $\bB_i$, $\bS_i$, $\bF_i$ and $\bD^i$ regions. Toward showing the above upper bound, we define two important events (which will depend on the draw $\boldf \sim \Dno$).

\begin{definition}
For a function $f \in \Dno$, we consider the following three events:
\begin{flushleft}\begin{itemize}
\item {\color{red} $\calE_1(f)$: This event occurs when there exists any node $v$ within the algorithm $\Alg$ such that 
    \begin{itemize}
    \item either the query $x_v$ lies in the region $D^{\ge q}$ defined by $f$, or
    \item the query $x_v$ satisfies $\|x_v\|_2\le \sqrt{n}-100q$ and lies in
      the region $D^{\ge 1}$ defined by $f$.
    \end{itemize}
}
\item $\calE_2(f)$: This event occurs if at the end of executing $\Alg$ 
   on the function $f$, there exist an $i\in [N]$ and two queries $x,y\in Q^q$\rnote{Minor: $Q^q$ or $Q^{q+1}$ --- isn't $Q^{q+1}$ the set of all $q$ queries the algorithm makes when the function is $f$? \color{red}Xi: Maybe it should be $Q^q$ since we start with $Q^0=\emptyset$ at the beginning.} that satisfy the following conditions:
   %produced by executing $\Alg$ on the function $f$, which satisfy the following two conditions:
\begin{itemize}
\item $Q^q\cap S_i$ 
\item There exists some $i \in [N]$ where $x, y \in S_i$ \blue{and $\|x\|_2, \|y\|_2 \leq \sqrt{n} + 1$}. 
\rnote{Do we want just the blue thing or do we want that $x,y \in \Shell$?}
\item The distance $\|x - y\|_2 \geq n^{1/4} (\log n)^2 \cdot \sqrt{q}$. 
\end{itemize}
\item $\calE_3(f)$: This event occurs whenever there exists two queries $x, y \in Q^q$ produced by executing $\Alg$ on the function $f$ where there is some $i \in [N]$ with $x, y \in S_i$, \blue{$\|y\|_2, \|x\|_2 \leq \sqrt{n} + 1$},\rnote{Here too, do we want just the blue thing or do we want that $x,y \in \Shell$?} and $f(x) \neq f(y)$.
\end{itemize}\end{flushleft}
\end{definition}

\begin{lemma}\label{lem:reject-and-3}
Suppose $\Alg$ is a deterministic $q$-query algorithm for testing convexity. Then, if $\Alg(f)$ outputs ``reject,'' the event $\calE_3(f)$ occurred.
\end{lemma}

\begin{lemma}\label{lem:ev3}
Suppose $\Alg$ is a deterministic $q$-query algorithm, where $q \leq ??$. Then, 
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \calE_3(\boldf) \wedge \ol{\calE_1(\boldf)} \wedge \ol{\calE_2(\boldf)} \right] = o(1).
\end{align*}
\end{lemma}

\begin{lemma}\label{lem:ev2}
Suppose $\Alg$ is a deterministic $q$-query algorithm, where $q \leq ??$. Then,
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \calE_2(\boldf) \wedge \ol{\calE_1(\boldf)} \right] = o(1).
\end{align*}
\end{lemma}

\begin{lemma}\label{lem:ev1}
Suppose $\Alg$ is a deterministic $q$-query algorithm. Then,
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf)\right] = o(1). 
\end{align*}
\end{lemma}

\begin{proof}
This lemma follows from a simple union bound. Note there are at most $2^q$ queries $x_v$ with $v \in \Alg$. Thus, we have:
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf)\right] \leq \sum_{v \in \Alg} \Prx_{\boldf \sim \Dno}\left[ x_v \in \bD^q  \right] \mathop{\lsim}^{(\ref{lem:exp-decrease})} 2^q \cdot 1/q! = o(1). 
\end{align*}
{\color{red}I hope the second part of $\calE_1$ follows from the discussion in
  the email thread on March 6.} \blue{Yup, I think this should be fine - it'll follow from the kind of calculations that will be in the proof of \Cref{lem:rad-by-rad}. Shivam and Rocco will fill this in.}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:one-sided} Assuming Lemmas~\ref{lem:reject-and-3},~\ref{lem:ev3},~\ref{lem:ev2},~\ref{lem:ev1}]
We upper bound the expression
\begin{align*}
\Prx_{\boldf \sim \Dno}\left[ \Alg(\boldf) = \text{``reject''}\right] &\mathop{\leq}^{(\ref{lem:reject-and-3})} \Prx_{\boldf \sim \Dno}\left[ \calE_3(\boldf)\right]  \\
		&\leq \Prx_{\boldf \sim \Dno}\left[ \calE_1(\boldf) \right] + \Prx_{\boldf \sim \Dno}\left[ \calE_2(\boldf) \wedge \ol{\calE_1(\boldf)}\right] + \Prx_{\boldf \sim \Dno}\left[ \calE_3(\boldf) \wedge \ol{\calE_2(\boldf)} \wedge \ol{\calE_1(\boldf)}\right] \\
		&= o(1),
\end{align*}
where the final line uses Lemmas~\ref{lem:ev3},~\ref{lem:ev2}, and~\ref{lem:ev1}.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:reject-and-3}}

\enote{This should be Xi's argument using the definition of convex hull, where we say that something has ``crossed the boundary''. Hopefully we can fill this in more formally...}

Since $\Alg$ is a $q$-query deterministic algorithm which has one-sided error, in order for the algorithm to output ``reject,'' it must produce a violation to convexity. The root-to-leaf path obtained by executing the algorithm $\Alg$ on a function $f$ leads to a set $Q^q$ where there are $x_1,\dots, x_{\ell}, y \in Q^q$ with $y \in \conv(x_1,\dots, x_{\ell})$, $f(y) = 0$ and $f(x_1) = \dots = f(x_{\ell}) = 1$. In particular, from $y\in \conv(x_1,\dots,x_\ell)$, we must have that, for any $u \in \R^n$, there exists some $j \in [\ell]$ where $\langle x_j, u \rangle \geq \langle y, u \rangle$. This implies that:
\begin{itemize}
\item We must have $y \in \Shell$. First, $\|y\|_2 \geq \sqrt{n} - 1$ since $f(y) = 0$. If $\|y \|_2 > \sqrt{n} + 1$, then letting $u = y / \|y\|_2$ would mean that there is some $x_j$ with $\langle x_j, u \rangle \geq \langle y, u \rangle > \sqrt{n} + 1$, and hence $f(x_j) = 0$, which would be a contradiction.

\item Next we must have $y\in B$.
Otherwise there exists an $i\in [N]$ such that $\langle y,g^i\rangle >r$.
Using $g^i$ as $u$ we have that there exists a $j\in [\ell]$ such that $\langle x_j,g^i\rangle \ge \langle y,g^i\rangle >r$, which implies that $f(x_j)=0$, a contradiction.

\item In addition, $f(y) = 0$ implies $y \notin B'$ by the definition of $f(y) = g_{\vec{H}, \vec{v}}(y)$ for $y \in \Shell$. In particular, there must be some index $i \in [N]$ so that $\langle x_j, g^i \rangle \geq \langle y, g^i \rangle > r - c_1 n^{1/4}$. Finally, we must have $\langle x_j , g^j \rangle \leq r$ as otherwise, $x_j \notin B$ and evaluates to $0$. For that setting of $j$, we must also have $\|x_j\|_2 \leq \sqrt{n} + 1$ since $f(x_j) = 1$. 
\end{itemize}
In summary, we must have both $\|y\|_2, \|x_j \|_2 \leq \sqrt{n} + 1$ and $x_j, y \in S_i$ for some $i \in [N]$. This concludes the proof.

\subsubsection{Proof of Lemma~\ref{lem:ev3}}

\enote{I'm hopeful this lemma will be straight-forward given the events. Essentially, we just need to ``randomize'' with respect to the action subspaces and perform union bounds only with respect to $q$.}

\subsubsection{Proof of Lemma~\ref{lem:ev2}}

\enote{I think this one will be the more complicated argument.}


